On the Utility of Domain Modeling Assistance with Large Language Models

Model-driven engineering (MDE) simplifies software development through abstraction, yet challenges such as time constraints, incomplete domain understanding, and adherence to syntactic constraints hinder the design process. This paper presents a study to evaluate the usefulness of a novel approach utilizing large language models (LLMs) and few-shot prompt learning to assist in domain modeling. The aim of this approach is to overcome the need for extensive training of AI-based completion models on scarce domain-specific datasets and to offer versatile support for various modeling activities, providing valuable recommendations to software modelers. To support this approach, we developed MAGDA, a user-friendly tool, through which we conduct a user study and assess the real-world applicability of our approach in the context of domain modeling, offering valuable insights into its usability and effectiveness.

==> sections/relatedWork.tex <==
\section{Related Work}\label{sec:relwork}

%\assignedto{Istvan}

\begin{comment}
    

     cognitive aspects of modeling
    \begin{itemize}
        \item~\cite{malinova2021cognitive}
    \end{itemize}
   model assistance  AND: Understanding the need for assistance in software modeling: interviews with experts ~\cite{savary2023understanding}\\
\end{comment}
Intelligent modeling assistants ~\cite{mussbacher2020opportunities}, are designed to support modelers during the early development phases such as analysis and design, by offering contextually relevant suggestions. In this section, we present an overview of current research in modeling assistants for Model-Driven Engineering (MDE).

A deeper understanding of the necessity for assistance in software modeling is crucial. To delve into this need, Savary-Leblanc et al. ~\cite{savary2023understanding} conducted interviews with experts. These experts provided feedback based on their practical experience with modeling languages and tools in industrial settings. From the qualitative analysis of these interviews, the authors extracted significant observations on how to design software assistants tailored for software modeling. These observations not only provide insights for tool vendors but also offer valuable guidance to the academic community, shaping the way we identify and design innovative solutions to assist modelers in their tasks. 

The complexity of systems is escalating, and the field of modeling is pressed to address this inherent complexity effectively. When addressing this, the focus shifts to the selection of suitable AI models for assistance tasks and the quality and availability of data for training these models. The options include using \textbf{pretrained} models trained on extensive datasets or \textbf{fine-tuning} them for specific software engineering tasks. Regardless of the approach, the dataset's quality and availability are paramount.  
%When addressing this, two critical aspects need to be considered: the selection of appropriate AI models for the assistance task and the availability and quality of the corpus or data used to train and feed these models. Regarding AI models, there are two main approaches: using \textbf{pretrained} models that have been trained on large-scale datasets or \textbf{fine-tuning} them specifically for software engineering tasks. Pretrained models offer the advantage of leveraging existing knowledge and language understanding, while fine-tuning allows customization and adaptation to the specific needs of the software engineering domain. However, regardless of the chosen approach, the availability and quality of the dataset play a critical role. Unfortunately, datasets in the software engineering domain are often scarce, and when available, they are not large enough to pre-train or fine-tune deep-learning models.
%For software modeling activities, several contributions were proposed to circumvent the lack of large datasets. The goal of these research contributions is to recommend domain concepts, their features, and relationships during modeling activities

In the current state of the art, three distinct perspectives have emerged, aiming to address the challenge of data scarcity. These perspectives focus on different levels of implementation and offer potential solutions to mitigate the problem, taking into account whether they train or utilize pretrained models or employ fine-tuning techniques.

The first perspective proposes embracing the limited amount of available models or metamodels and using them to train recommender systems. 
%Di Rocco et al.~~\cite{RoccoSRN21} proposed an approach based on graph kernels that only need a small-size dataset for training. Although the results were promising, the quality of the recommended elements remains too low to be used in real settings.
 Weyssow et al.~~\cite{weyssow2022recommending}, gathered a dataset of models and metamodels relevant to the target objective and applied appropriate transformations to obtain textual formats and then train an LSTM neural network. The authors obtained limited results, especially when applied to the iterative construction of a metamodel.
Other techniques of model completion do not involve sophisticated neural network models and use similarity criteria to suggest elements that are similar to the item being modified. This is the work of Elkamel et al. ~\cite{elkamel2016uml}, which proposes related UML classes from a source of UML class diagrams. Using a clustering algorithm that classifies a set of UML classes into a large number of similar groups, the authors were able to index this dataset and use it to suggest related items. 


 From a second perspective, Capuano et al. ~\cite{capuano2022learning} trained a model recommender with data extracted from Java projects but they used document embedding techniques to abstract a set of domain concepts and suggested to the designer the most similar documents.   
 Similar to this work, Di Rocco et al. ~\cite{rocco2021gnn}, exploited the available large code bases to reverse-engineer a set of models to train a RoBERTa language model. The results are acceptable, but the reverse-engineered models on which the authors had to rely for training led to suggestions that reflect implementation aspects rather than the modeled domains.




The third perspective is to exploit what is already encoded in natural languages. 
Arora et al.~\cite{arora2016extracting} 
propose an approach to automatically extract domain models from natural-language requirements using dependency parsing and rule-based techniques. The study shows that the proposed approach is effective in extracting domain models from requirements documents  can be useful for specifying the system under development. According to expert
evaluation, the extraction rules in their implementation
achieve correctness between $74\%$ and $100\%$. 
Saini et al.~~\cite{saini2022automated} proposed a bot to assist modelers with the creation of domain models from requirements expressed in natural language using a combination of NLP techniques. For learning the context information, the authors used a pre-trained Bidirectional Long Short Term Memory (BiLSTM) neural network. Although their results show that the bot can be useful, they did not exploit LLMs, which we believe will positively impact predicting new modeling elements.  With the same  goal of exploiting knowledge captured in general and specific natural-language documents,  
Burgueño et al.~~\cite{burgueno2021nlp} exploited these documents to train language models to suggest model completions. 
All the aforementioned approaches have been custom-designed from the ground up for specific modeling or specific modeling formalism, resulting in significant time and effort required for their development (e.g., limited reusability) and integration. This is in stark contrast to the approach we introduce in our work ~\cite{chaaben2022}, which demonstrates a more adaptable and potentially more efficient methodology.
Our approach aims then to harness the richness of natural language, enabling more robust and versatile applications in modeling assistance.   


A recent development in the field by Clariso et al. ~\cite{clariso2023model} presents an innovative application of model-driven engineering to support the prompt engineering process. This work proposes using a domain-specific language (DSL) to define platform-independent prompts, which can then be adapted to generate high-quality outputs in target AI systems. This methodology aligns with our focus on leveraging natural language for modeling assistance, emphasizing the importance of well-crafted prompts in achieving effective AI-driven model completion.



==> snippets/4-approach-old.tex <==
\section{Prompting LLMs for Domain Model Completion: Running Example}\label{sec:approach}

%\lola{My idea is:  1) to have a very short introduction to an example where we present a model under construction (running example, ie previous section).
%2) In the approach section, we say how we create the prompts in a generic way and we use the running example to illustrate some prompts (like we did in our ICSE NIER paper).
%3) We explain how we parse the outcome of the LLM in a generic way and show it with the running example
%4) we present the postprocessing phase and again we use the running example to illustrate it.
%5) Finally, using the running example again, we present the suggestions that we would offer to the user (Figures 1b, 1c, 1d)}

%\houari{To conduct our study, we propose an approach and a tool for domain modeling assistance using LLMs.}
In this section, we present our approach to model completion through LLMs. Later, we illustrate the approach using the following running example.





% \lola{I would finish here the running example subsection and I will present the rest. I would only show Figure 1a as part as the running example.}



%Since this modeling activity is strongly bounded by the domain, a modeler who has limited knowledge of it may encounter some difficulties. Thus, we propose a recommender system that leverages a powerful AI technique to address these challenges. 

%The following subsection describes in detail the generalizable approach we follow to building an efficient tool for assisting modelers during one particular task, domain modeling and that is potentially adaptable to various other formalisms.


%\subsection{Overview of the approach}

Our approach involves exploiting the large amount of learned general knowledge contained within the LLMs instead of relying on collecting domain-specific data and training a new model or fine-tuning a pre-trained one. In order to use the data encrypted in LLMs, we rely on semantic mappings. Therefore, we introduce a new paradigm for extracting knowledge from text and aligning it with elements in modeling formalisms and reciprocally.

%This method serves as a crucial bridge, allowing the system to not only comprehend but also eventually build meaningful representations within the modeling formalism. \lola{I am not so sure what this last sentence wants to communicate here. If we want to mention this, how about we do it later? even as late as in the conclusions. I think, since we haven't introduced the approach yet, this will confuse the reader}
%This dynamic process facilitates the transformation of linguistic complexities and contextual insights from natural language into a structured framework, thereby seamlessly integrating textual comprehension with formal representation.

 \begin{figure}[H]
\centering
\includegraphics[width=1\columnwidth]{figures/approach.pdf}
\caption{Illustrating iterative steps in Model Completion- \href{https://drive.google.com/file/d/1nS9m5s4wW0zS87plmU-Mou-wFgCRGZOQ/view?usp=sharing}{figures link } \id{A legend would be required. What is the difference between the two arrows? What is dashed vs solid line rectangle?}}


\label{fig:approach}
\end{figure}
\todo{ update legend; semantic mapping, data flow, text}
%\id{I don't see how \figref{fig:approach} corresponds to the structure of the section/paper. A good overview figure would lead the reader to the right section headers. Also unreadable. Font size should be similar to the text's size to reduce the cognitive effort of reading. Let's work on this.}

Figure~\ref{fig:approach}  presents an overview of the proposed approach, which is applied in an \textit{ \textbf{iterative}} manner to allow for continuous refinement and completion of the model. 

Starting from a partial model (a.k.a. model under construction), the first step is to consider  the textual representation of graphical models or its textual serialization (e.g., for XMI, UML or Ecore models), and use parsers to automate the extraction of information. We use the obtained information and build a \textbf{semantic mapping}, defined as the translation of elements within the domain model under construction into semantically equivalent text. This text is then seamlessly integrated into the prompt, ensuring its comprehensibility to the AI agent at a later stage.

As a community effort, generative AI users have created several guidelines for creating good prompts for typical tasks, \cite{PromptingGuide2023,liu2022design}. In this methodology, we incorporate these principles to meticulously craft prompts tailored to our objectives. Each prompt  is composed of three critical elements: the \emph{Instruction} outlining the task at hand, \emph{Few-shot examples} providing context and guidance, and the \emph{encoded model under construction}, all aimed at facilitating the completion of the model.

We query a generic LLM using the designed prompt to \textbf{predict} elements that are missing from a partial model. Following this, we apply a second \textbf{semantic mapping} to the generated text to extract potential  relevant elements.  These elements are then presented to the user, who can \textbf{select} and incorporate the most relevant ones into the partial model as deemed appropriate.
Depending on the nature of the suggestions that we would like to provide, 
%(for instance new entities, attributes, associations in a class diagram), 
we need to adapt our semantic mappings. In the following, we will provide all the details and we illustrate them using our running example.
%these two semantic mappings and provide information of the prompts that we build.

%Our approach covers two types of modeling languages: static models, i.e., UML class diagrams; and dynamic models, i.e., UML activity diagrams. By considering multiple formalisms, we aim to gain a more nuanced understanding of our method’s performance, applicability, and generalizability. 
%\lola{We should not say anymore that we ``illustrate'' our approach. Since this is a journal paper, the work is supposed to be mature. And in fact, it is, as it is even supported by a tool. I am not so sure, however, whether we should talk about activity diagrams here. Let us discuss this in our next meeting.}



%\subsection{Class Diagram Completion}

%\id{I don't get the relationship of this subsec to the overview. This would make sense if there was another subsec about completing other diagrams. In essence, 3.2 is the instantiation of 3.1. A better title would be needed at least, to make this more natural. Also, in Fig 1, you already show a class diagram, so in 3.1 you are assuming 3.2.}

%\id{It must argued at this point right here, why recommending names-attributes-associations is enough.}

%\subsection{Running example}

\id{Section/subsection headers are off}\MBC{Resolved?}\id{I'd still recommend an unnumbered paragraph$\ast${} here that says ``Running example''.}

%We simulate a modeler who is specifying a domain model of a hospital system, and at a certain point in time, due to either the complexity of the required task or the lack of experience, she does not know how to proceed; she may be unsure about which concept to add to the canvas or the appropriate type of association between two classes, for instance. 
%In this respect, domain model assistance is expected to help enhance the specification of the partial model under construction by recommending a useful list of new modeling elements.

Let us assume that a modeler is building a domain model to capture information about hospitals. At a certain point in time, the model is in the state that Figure~\ref{fig:runningExample} captures. It has only 3 basic concepts, \texttt{Hospital}, \texttt{Staff} and \texttt{Doctor}. A hospital has an attribute of type String named \texttt{name}, one other attribute \texttt{rooms number} of type int and one aggregation to the entity \texttt{Staff}. \texttt{Staff} has one attribute \texttt{name}, while \texttt{Doctor} has two  attributes \texttt{speciality} and \texttt{qualification}.


 \begin{figure}[h]
\centering
\includegraphics[width=0.4\columnwidth]{figures/modelunderconstruction1.pdf}
\caption{Hospital domain model (in construction)}
\label{fig:runningExample}
\end{figure}
In the process of domain modeling, achieving a comprehensive representation necessitates identifying the entities involved and understanding their roles and responsibilities within the system (class names), the characteristics of these entities (attributes), and how they interact with each other (associations). Our approach is precisely aimed at enriching the domain model by  suggesting class names, attributes, and associations. 

 
\subsection{Class names suggestions}

%\id{Terminology should be more precise. Is it suggestion or recommendation?}


%We focus first on how we design our completion system to suggest entities, i.e., new classes. The core of our approach centres on creating a thoughtfully designed prompt, which plays a key role in guiding our model's completion process. 

When creating the semantic mapping between models and prompts for class name suggestions, we combine three essential components within the prompts: the task description,  a small number of shots or examples, and the text to complete, as depicted in Figure ~\ref{fig:approach-concepts}.

Regarding class name suggestion, we include within the prompt the text '\textit{Generate related concepts}' as the task description. 
Then, we provide the LLM with a set of shots or examples that act as guides for the LLM's reasoning process. They enable the model to generalize from the presented instances and make informed predictions about the relationships, connections, and concepts that are likely to exist within the partial domain model.
More specifically, we use existing diagrams from diverse and unrelated domains to craft these examples. 



%As shown in Figure~\ref{fig:approach-concepts}
First, we add to our prompt the package name (X) to establish the contextual backdrop of this domain mode, then we add pairs of related classes (i.e Y and Z, where Y and Z are connected with a relationship). and, we define a syntactic pattern where we introduce the relationship between two related elements by means of representing them between square brackets. 
Subsequently, a shot will follow the following syntax: X: [Y,Z], [Z,C]... In the final step, we build a query from the partial domain model under construction. To do this, we select between 2 and 4 pairs of related classes, put the classes' names in square brackets, and add them to the prompt. In Figure~\ref{fig:approach-concepts}, we show an example where we partially encode two distinct diagrams: the \textit{Banking System} and the \textit{Reservation System}. Following the described methodology, for each shot or example, we include some related concepts with the intention of guiding the engine in this particular task. 
Finally,  under ``Generated text'' we can observe the highlighted text that has been generated to complete the \textit{Hospital System}. 



\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/concepts.pdf}
\caption{Completion of Hospital Domain Model: Class Names Integration }

%\id{Can't read the figure---increase font size. Semantics of arrows unclear. Legend shows a roundtangle, figure has rectangles, also a highlight in a similar (same?) color.}

\label{fig:approach-concepts}
\end{figure}
Once the LLM has generated the text corresponding to our prompt, we apply a string-searching algorithm to the generated text to extract relevant class names and the association that exists between them ([STEP 3] of our approach). Next, we put in place a post-processing phase in which we remove spelling errors and noisy data such as digits, which are usually not part of domain models. After this step, we obtain the potential missing classes (and associations between them). In our example, these are \texttt{Patient, Appointment} and \texttt{Address}.  These suggested classes are then presented to the user after ensuring they are not already present within the canvas.   %as shown in Figure~\ref{fig:approach-concepts} with a red color. % In section~\ref{subsubection:Associations} we explain how we consider the suggested relationships between the new concepts and introduce them in the model under construction. 
One can notice that for this example, all the suggestions are closely related to the Hospital domain that is being modeled, which is the desired behavior.

Our engine follows a ranking strategy to suggest new elements. We create different prompts and query the LLM several times. All these prompts share the same few shots but different queries, each query containing a different subset of model elements from the partial model. As a result, we obtain for each prompt a set of suggested concepts. Then, all the obtained concepts from the different prompts are ranked by their frequency, from higher to lower. Only those concepts with higher frequency are suggested to the user.

\subsection{Attributes suggestions}
\begin{figure}[t]
  \centering  \includegraphics[width=0.9\columnwidth]{figures/attributes.pdf}
  \caption{Completion of Hospital Domain Model: Attributes  Integration}
  \label{fig:approach-attributes}
\end{figure}



Similar to class names suggestions, we provide few examples that serve as guidance for the task of suggesting potential missing attributes.
As illustrated in Figure ~\ref{fig:approach-attributes}, we consider actual class diagrams and we concatenate the package name and existing class names with their attributes in square brackets, ending with the class for which we are finding potential attributes.  
Adopting a similar strategy to that used for class name recommendations, we use a frequency-based ranking function that takes as input all the text generated by GPT-3 for different prompts. Then, we generate attribute suggestions using those concepts that are at the top of the ranking. We showcase in Figure~\ref{fig:approach-attributes} the resulting text for the different classes in the model under construction.   For instance, for the class \textit{Patient}, we have obtained \texttt{name, phoneNumber} and \texttt{id} as potential missing relevant attributes.  To obtain the type of each suggested attribute, we perform a  second iteration. This involves utilizing prompting once again in conjunction with the powerful generative model. 

%The process of completing the typing of each attribute involves providing the engine or LM with a set of attribute names along with their associated types. Then, to determine the relevant type for a specific attribute, we prompt the LM by providing the attribute name for which we want to know the type. By leveraging this information, the LM generates a response that recommends the most suitable type for the specified attribute.



\subsection{Associations suggestion}
\label{subsubection:Associations}

Regarding the suggestion of association names, we design our prompt as follows: from unrelated diagrams, we select pairs of classes that have an association between them.  Each pair of classes is used to build a shot by concatenating the name of the classes and the name of the association. 
Similarly, when it comes to the suggestion of association types, our prompt is designed as follows: from unrelated diagrams, we select pairings of classes with an association.  Each pair of classes is used to construct a shot by concatenating the class names and the association type. Figure~\ref{fig:approach-association} represents the completed model after going through the semantic mapping step to extract the knowledge (type and name of associations) and introduce them to the model under construction. 



\begin{figure}[t]
  \centering
  \includegraphics[width=1\columnwidth]{figures/associations.pdf}
  \caption{Completion of Hospital Domain Model: Associations Integration}
  \label{fig:approach-association}
\end{figure}

    \begin{comment}

        \subsection{Applicability across different formalisms }
Not only static formalisms
\id{This doesn't belong here. Say something about generalizability in the intro and then address the question in detail when you talk about the threats to external validity.}

\id{In general, a good paper flows naturally. You don't want to bother the reader with these sidebars, just allow them to rapidly proceed to the core of the paper.}
    \end{comment}


==> snippets/background.tex <==
\iffalse

\subsection{Software Modeling}

The complexity of modern software systems often requires rigorous formal engineering methods. Pertinent examples include cyber-physical systems, especially of safety-critical nature, such as automotive systems.
Model-driven engineering (MDE)~\cite{schmidt2006guest} advocates modeling software systems before they get realized, and use these models for an array of crucial engineering activities, including requirements formalization ~\cite{dromey2003requirements}, rapid prototyping and validation ~\cite{moeskopf2008introduction}, formal verification of functional ~\cite{gonzalez2014formal} and extra-functional properties, and code generation ~\cite{kelly2008domain}.

Within MDE, \emph{domain modeling}~\cite{iscoe1991domain,prieto1991domain} focuses on externalizing core domain concepts and relationships among them, typically relying on a subset of the UML Class Diagram notation~\cite{berardi2005reasoning}. Class diagrams have shown to be a balanced combination of sufficient descriptive power and economical notation, allowing for an efficient modeling experience~\cite{lindland1994understanding}.

%Through the strategic application of conceptual modeling principles ~\cite{lindland1994understanding}, domain modeling provides a detailed blueprint of domain-specific entities, facilitating a comprehensive framework for software design. 
%Metamodel

%In order to define the languages used to create a model whithin any modeling formalism, including domain models, the concept of \emph{metamodeling} emerges as a critical facilitator in MDE\cite{nordstrom1999metamodeling}, providing a structured framework. A metamodel, in essence, is a '''model of models'''; it specifies the abstract syntax, semantics, and constraints necessary for constructing and validating models.   


% Why modeling assistance
Recognizing the critical role of domain modeling in software system development and acknowledging that it is a challenging and time-consuming task requiring expertise and experience, this paper focuses on helping modelers in this process. While modeling assistance generally aims to enhance adherence to syntactical rules, best practices, and alignment with constraints and metamodels, our work specifically focuses on ways to provide modelers with relevant and impactful content. We delve into assessing the effectiveness and utility of the proposed assistance, aiming to significantly streamline the domain modeling task. 

Addressing the challenges of manual software modeling is characterized by its time-consuming nature and susceptibility to errors, which underscores the importance of assistance in this domain.
\todo{Istvan.}

\id{Pain point: software modeling is hard by hand. Manual labor is error-prone and costly. The human needs assistance to create better models more efficiently. This is basically what you describe here, but the link with our work is not natural. The natural answer to the problems is the next subsection: assistance.}

\fi




%Saini et al.~~\cite{saini2022automated} proposed a bot to assist modelers with the creation of domain models from requirements expressed in natural language using a combination of NLP techniques. For learning the context information, the authors used a pre-trained Bidirectional Long Short Term Memory (BiLSTM) neural network. Although their results show that the bot can be useful, they did not exploit LLMs, which we believe will positively impact predicting new modeling elements.


%To further improve these models' ability across different tasks, fine-tuning is a common employed technique. 
%Fine-tuning involves adjusting the pre-trained model's parameters slightly to make it more adept at a particular task. This process typically requires a smaller, task-specific dataset on which the model is further trained.
%However, it faces two major issues: \textit{the process can be computationally demanding}, and \textit{there may be insufficient training data for certain tasks}. In contrast, prompt learning bypasses these challenges by using training examples as input, rather than updating parameters. 
%While many prompt learning approaches exist for LLMs ~\cite{liu2023pre} like the zero-shot technique,   the chain of thought (CoT) technique ~\cite{wei2022chain} and the Generated knowledge prompting ~\cite{liu2021generated},
%we focus on the \emph{few-shot learning}.
%This approach involves presenting the model with a small number of example inputs that illustrate the task at hand, effectively guiding the model to understand and execute similar tasks.
%Unlike traditional training methods that require substantial modifications to the model's parameters, few-shot learning operates by leveraging the model's pre-existing knowledge and capabilities, instructing it to apply this knowledge in new, specific contexts based on the examples provided.

==> snippets/tool-old.tex <==

\begin{comment}
    
\subsection{Developing a DSM Graphical Editor for class diagrams }

\label{sec:toolsupport}
To implement our approach we thought about generating a tool for our own Domain Specific Language, i.e a Graphical Editor for completing class diagrams.
Creating a DSL in the Model-driven Engineering context is often called Domain-Specific Modeling (DSM). By employing the Eclipse platform, specifically the Sirius plugin~\cite{websiteEclipse}, we leverage the powerful capabilities of these tools to construct our DSL-based graphical editor. In fact, Sirius offers a solution for the quick development of graphical tools without any knowledge of the backend procedures and is very flexible and adaptable\cite{viyovic2014sirius}. Obeo, the firm that developed Sirius, offered a list of best practices\cite{siriusBestPractices} that we adhered to, in order to assure better performance.


To create this tool, we follow several key steps. First, we generate a metamodel using EMF Ecore, which defines the structure and behaviour of the editor. The metamodel serves as a formal representation of the tool's concepts and their relationships, enabling visualization and manipulation of class diagrams. Figure~\ref{fig:metamodel} illustrates the structural meta-model, showcasing the incorporated features and elements.
\MBC{to be discussed}
Next, we define notations for the editor by creating a Sirius representation model that serves as a  mapping between the metamodel elements and the graphical representations, such as shapes, colors, and connections, establishing the visual appearance of the editor.
This mapping is typically defined through the ODesign file, short for "Sirius Object Designer" file. It contains configurations, rules, and instructions that link the elements of the metamodel to their corresponding graphical representations.
\MBC{not sure if we put details about the metamodel, therefore an illustrative figure}
For instance, in our ODesign file, we ensure that class elements, depicted in the metamodel by the UML class "Clazz" (\ref{fig:metamodel}), are represented as rectangles with grey colors and we orchestrate the placement of the attributes elements within these rectangular class elements.

We also specify the behavior of the editor, encompassing various editing capabilities like adding, deleting, and modifying elements. 
Our careful configurations of the ODesign file contribute to a unified and intuitive user experience.

Finally, we generate the necessary code and configurations to bring the editor to life, ensuring that it is fully functional according to some specified specifications. Throughout this process, we incorporate custom code to modify the editor's behavior to align with specific requirements and constraints, thus enhancing its functionality and adaptability.

\todo{ a figure to illustrate steps and important files in Sirius project }


\todo{a figure for metamodel ? not sure if necessary }
\subsection{Recommendation engine}
The next step is to create the recommendation module.
For our task of class diagram completion, we specifically take advantage of GPT-3, which is one of the most powerful LLMs---it contains 175 billion parameters~\cite{brown2020language}---, to represent most of the existing general concepts to support software specialists when modeling. 
\todo{ More details ... parameters, frequency-based selection ... }
 In order to integrate it seamlessly with the existing Java-based editor, we utilize Java code for making the API calls to OpenAI\footnote{https://platform.openai.com/playground}. Although OpenAI's API does not provide specific Java code for these calls, we leverage a different plugin\footnote{https://github.com/TheoKanning/openai-java } that allows us to avoid the need for integrating Python scripts and ensures both compatibility and efficiency.
\subsubsection{Recommendation modes}


MAPLe offers three distinct recommendation modes: Recommendation On Request, Automatic, and Recommendation at the End. These modes cater to different user preferences, allowing for either active engagement or passive suggestions during the modeling process.

In the \textbf{Recommendation On Request Mode}, the user has the flexibility to request specific types of predictions during the modeling process. This mode allows him to actively seek potential attributes, concepts, or associations based on his needs.
%As shown in figure~\ref{subfig:onRequestMode}, with a right click on a specific class in the canvas, a list of attributes to that class will be shown to choose from and be added to the model under construction. 
    
 In the \textbf{Automatic Mode}, suggestions for concepts and operations are continuously provided as the modeling process unfolds. Whenever elements are added to the model under construction, an implemented algorithm triggers the suggestion of relevant elements. The canvas displays two lists, each containing suggestions for a specific type of element, as illustrated in the accompanying figure~\ref{subfig:automatic}. These suggestions aim to assist modelers by offering timely recommendations that align with the ongoing modeling context. 

 The \textbf{ Recommendation at the End Mode} is a mode that allows users to evaluate their completed modeling task and receive suggestions on any missing elements as a final step. In this mode, the user simply clicks on a button labelled "predict" when he believes he has finished the modeling process. The system then generates a list of suggestions that includes concepts, attributes, and associations for each class present in the canvas. This list is displayed to the user, who can then select the desired suggestions to incorporate into the initial model.


%It is worth noting that, while conducting   the user study, we asked the participants to complete a free task where they have the flexibility to toggle between different modes or choose not to select any specific mode



\end{comment}




\iffalse

\begin{longtable}
{@{}p{2cm}p{2.5cm}p{2.5cm}p{3cm}p{2.5cm}p{4.5cm}p{4.5cm}@{}}

\caption{Example from a Log CSV File} \\
\toprule
Timestamp           & Recommendation-Mode & Operation                 & Classes on Canvas          & Suggested Classes & Attributes for Canvas Classes       & Attributes for Suggested Classes \\
\midrule
\endfirsthead
\multicolumn{7}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
Timestamp           & Recommendation-Mode & Operation                 & Classes on Canvas          & Suggested Classes & Attributes for Canvas Classes       & Attributes for Suggested Classes \\
\midrule
\endhead
\bottomrule
\endfoot
\bottomrule
\endlastfoot

2023-05-08 12:00:43 & Automatic-Mode      & Accept Concept From view  & \{ Student \}              & School, Teacher   & Student: []                            & School: [], Teacher: [], Student: [] \\
2023-05-08 12:01:02 & Automatic-Mode      & Create attribute          & School, Teacher, Student   & Course, Course    & School: [], Teacher: [], Student: [address] & student: [firstName, lastName, placeOfBirth, address, gender, level, middleName, dateOfBirth], course: [] \\
\end{longtable}

\fi



Every record is labeled with a \textit{timestamp} 
\begin{itemize}
    \item Timestamp: The exact moment an action occurs, precise to milliseconds.
    \item Recommendation Mode: The selected prediction mode. 
    \item Operation: Actions performed by the user, like adding or deleting elements, or accepting suggestions.
    \item Classes on Canvas:  Names of model classes currently displayed to the user.
    \item Suggested Classes: Classes recommended by the system for potential inclusion in the model. 
    \item Potential Attributes for Canvas Classes: Attributes considered for each class on the canvas.
    \item Potential Attributes for Suggested Classes: Attributes considered for each class in the suggestion list.
    \item Potential Associations for Canvas Classes: Possible relationships between classes on the canvas.
    \item Potential Associations for Suggested Classes: Possible relationships between classes in the suggestion list.
\end{itemize}



%Sirius, operating as a language workbench within the Eclipse platform, is tailored for graphical modeling languages. It leverages the data models created by EMF to produce visual representations, which are key for user interaction with the models.

%If we want it brief: 
% Sirius provides the means to define how these models are visually represented and interacted with, turning the abstract data structures of EMF into concrete, user-friendly graphical elements.
% If we re looking for details: 
%Furthermore, Sirius offers an efficient solution for the quick development of graphical tools and allows for the creation of a representation model. This model acts as a mapping between the metamodel elements and the graphical representations like shapes, colors, and connections, thus establishing the visual appearance of the editor. 
% Such mapping is typically defined through the ODesign file, which contains configurations, rules, and instructions that link the elements of the metamodel to their graphical representations. For instance, class elements in the metamodel are represented as rectangles in specific colors, with attributes placed strategically within these shapes.


==> tables/design.tex <==
\begin{table}[h]
\centering
\begin{tabular}{ll|lll|l}
\cline{3-5}
 &  & \multicolumn{3}{c|}{Domain} &  \\ \cline{3-5}
 &  & \multicolumn{1}{c|}{D1} & \multicolumn{1}{c|}{D2} & \multicolumn{1}{c|}{D3} & \textit{Sample size} \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Recommender\\ mechanism\end{tabular}}} & RR & \multicolumn{1}{l|}{G1 (n = 5)} & \multicolumn{1}{l|}{G2 (n = 5)} & G3 (n = 5) & \multicolumn{1}{c|}{15} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & AR & \multicolumn{1}{l|}{G2 (n = 5)} & \multicolumn{1}{l|}{G3 (n = 5)} & G1 (n = 5) & \multicolumn{1}{c|}{15} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & FR & \multicolumn{1}{l|}{G3 (n = 5)} & \multicolumn{1}{l|}{G1 (n = 5)} & G2 (n = 5) & \multicolumn{1}{c|}{15} \\ \hline
 & \textit{Sample size} & \multicolumn{1}{c|}{15} & \multicolumn{1}{c|}{15} & \multicolumn{1}{c|}{15} &  \\ \cline{3-5}
\end{tabular}
\caption{Experimental design}
\label{tab:design}
\end{table}

\

==> tables/metrics.tex <==
\begin{table}[h!]
\centering
\caption{Summary of Metrics Used in the User Study}
\label{tab:metrics_summary}
\begin{tabular}{@{} lll @{}}
\toprule
\textbf{RQ} & \textbf{Metric} & \textbf{Domain} \\ \midrule
RQ1 & Mean time to complete task & Performance Metrics\\
& Number of experiments completed in time & Performance Metrics\\
RQ2 & Acceptance Rate & User Interaction Metrics \\
& Contribution Rate & Quality Assessment \\
RQ3 & Overlap Coefficient & Model Diversity \\
RQ4 & Mode Utilisation Frequency & Tool Usage \\
RQ5 & Modeling Experience Evaluation & User Feedback \\
\bottomrule
\end{tabular}
\end{table}

==> tables/participants.tex <==
\begin{table}
\centering
\begin{tabular}{@{}ll|ccc|l@{}}
\cmidrule(lr){3-5}
& & \multicolumn{3}{c|}{Domain} & \\ \cmidrule(lr){3-5}
& & \multicolumn{1}{l|}{D1} & \multicolumn{1}{l|}{D2} & \multicolumn{1}{l|}{D3} & \begin{tabular}[c]{@{}l@{}}Sample\\  size\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Recommender\\ mechanism\end{tabular}}}  & Automatic & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{10} & 10 & \multicolumn{1}{c|}{30} \\ \cmidrule(l){2-6} 
\multicolumn{1}{|l|}{} & At-End & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{10} & 10 & \multicolumn{1}{c|}{30} \\ \cmidrule(l){2-6} 
\multicolumn{1}{|l|}{} & On-Request & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{10} & 10 & \multicolumn{1}{c|}{30} \\ \midrule
& Sample size & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{30} & 30 & \\ \cmidrule(lr){3-5}
\end{tabular}
\caption{Distribution of participants across domains and recommender mechanisms}
\label{tab:participant_distribution-old}

\end{table}

==> tables/tasks.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|}
\hline
Group & Task Order \\
\hline
Group 1 & Automatic → At-End → On-Request \\
Group 2 & At-End → On-Request → Automatic \\
Group 3 & On-Request → Automatic → At-End \\
\hline
\end{tabular}
\caption{Task order for each experiment group.}
\label{tab:task_order-old}

\end{table}

